Representational aspects of depth and conditioning in normalizing flows

Normalizing flows are among the most popular paradigms in generative modeling, especially for images, primarily because we can efficiently evaluate the likelihood of a data point. This is desirable both for evaluating the fit of a model, and for ease of training, as maximizing the likelihood can be done by gradient descent. However, training normalizing flows comes with difficulties as well: models which produce good samples typically need to be extremely deep -- which comes with accompanying vanishing/exploding gradient problems. A very related problem is that they are often poorly conditioned: since they are parametrized as invertible maps from $\mathbb{R}^d \to \mathbb{R}^d$, and typical training data like images intuitively is lower-dimensional, the learned maps often have Jacobians that are close to being singular. In our paper, we tackle representational aspects around depth and conditioning of normalizing flows: both for general invertible architectures, and for a particular common architecture, affine couplings. We prove that $\Theta(1)$ affine coupling layers suffice to exactly represent a permutation or $1 \times 1$ convolution, as used in GLOW, showing that representationally the choice of partition is not a bottleneck for depth. We also show that shallow affine coupling networks are universal approximators in Wasserstein distance if ill-conditioning is allowed, and experimentally investigate related phenomena involving padding. Finally, we show a depth lower bound for general flow architectures with few neurons per layer and bounded Lipschitz constant.

==> conclusion.tex <==
\section{Conclusion} 

In this paper, we initiated a theoretical study of representation aspects of flow models, providing separations with non-invertible models like GANs, and studied the limitations of a popular architecture based on affine coupling blocks. 

Given the popularity of both families of models, we hope this paper will serve as an initiation of a richer study on the comparative benefits for different deep generative models, both from the representation theoretic and algorithmic aspects. 

==> linsim.tex <==
\section{Missing proofs from Section~\ref{s:linsim}}
\label{a:linsim}

\subsection{ Proof of Lemma \ref{lemma:simulate_swap}}
Choose a swap by fixing some $i$ and $j$. We can construct it as follows. Let $g$ be a scaling of $i$ by $-1$, $f$ be a shear from $j$ to $i$ by $1$, and $h$ be a shear from $i$ to $j$ by $-1$. Then $f\circ h \circ f\circ g$ can be seen as the matrix multiplication (only viewing the $i$th and $j$th basis vectors)
\begin{equation*}
    \begin{bmatrix}1 & 1\\0 & 1\end{bmatrix}
    \begin{bmatrix}1 & 0 \\ -1 & 1\end{bmatrix}
    \begin{bmatrix}1 & 1\\0 & 1\end{bmatrix}
    \begin{bmatrix}-1 & 0\\0 & 1\end{bmatrix} = \begin{bmatrix}0 & 1\\1 & 0\end{bmatrix}.
\end{equation*}
This clearly swaps $i$ and $j$.

\subsection{Proof of Lemma \ref{l:mainlin}}
Consider a scaling of a coordinate $i \in [d+D]$ by $c \in \mathbb{R}$ first. If $i \leq d$ then we can let $B = I$ and $C$ a diagonal matrix, s.t. 
$C_{ii} = c$ and $C_{jj} = 1$, if $j \neq i$.  
The case $i > d$ is analogous.  
%If $i > S$, then we can let $C = I$ and $B$ a diagonal matrix with all ones except at the $i - D$th element, which is $c$. 
%In either case, multiplying out the matrices in the statement gives a diagonal matrix with all ones on the diagonal save the $i$th element of $c$, which is exactly as desired.

Next consider a shear from $j$ to $i$ by $c$ for some $i, j, c$. There are two cases. First, consider the case where both $i \leq d$ and $j \leq d$ or both $i > d$ and $j > d$. Without loss of generality, let's assume $i \leq d$ and $j \leq d$ (the argument is symmetric for the other case). We'll use the notation $(x_i)_j$ to mean a vector that is all zeros except the $j$th coordinate which has value $x_i$.

Consider the first ordering of the 3 matrices from the lemma statement, and let $E$ be all zeros with a $1$ in the $j$th column and top row. Then for some $x \in \R^d$, $y\in \R^D$,
\begin{equation*}
    \begin{bmatrix}
    I & 0 \\ E & I
    \end{bmatrix}
    \begin{bmatrix}x \\ y\end{bmatrix} = \begin{bmatrix}x\\y + (x_j)_1\end{bmatrix}.
\end{equation*}
Let $D$ be all zeros with a $c$ in the first column and $i$th row. Then
\begin{equation*}
    \begin{bmatrix}I & D\\0 & I\end{bmatrix}\begin{bmatrix}x\\y + (x_j)_1\end{bmatrix} = \begin{bmatrix}x + (cx_{j})_i\\y + (x_j)_1\end{bmatrix}.
\end{equation*}
Let $A = -E$. Then
\begin{equation*}
    \begin{bmatrix}I & 0\\-E & I\end{bmatrix}\begin{bmatrix}x + (cx_{j})_i\\y + (x_j)_1\end{bmatrix} = \begin{bmatrix}x + (cx_{j})_i\\y\end{bmatrix}.
\end{equation*}
This is precisely a shear from $j$ to $i$ by $c$.
If we did the same thing with the bottom $3$ matrices we cover the $i > d$, $j > d$ case.

Next, consider $i > d$ and $j \leq d$ or $i \leq d$ and $j > d$. Without loss of generality, consider the case $i > d$ and $j \leq d$ (the other is symmetric). Using the first ordering of the 3 matrices in the lemma statement, let $E$ be all zeros with a $c$ in the $(i - D)$-th row and $j$-th column and let all other matrices be zeros. Then, dropping the identity matrices, we get
\begin{equation*}
    \begin{bmatrix}
    I & 0\\ E & I
    \end{bmatrix}
    \begin{bmatrix}
    x\\y
    \end{bmatrix}
    =
    \begin{bmatrix}
    x\\
    y + (x_j)_{i - D}
    \end{bmatrix}.
\end{equation*}
This is precisely the desired shear, completing the proof of the lemma.  %Again, we can easily run the same argument for the flipped case using the matrix containing $H$ instead.
%This shows that we can construct any shear or scaling as desired.


==> old_introduction.tex <==
\section{Introduction} 

Deep generative models are one of the lynchpins of unsupervised learning, underlying tasks spanning distribution learning, feature extraction and transfer learning. Parametric families of neural-network based models have been improved to the point of being able to model complex distributions like images of human faces. One paradigm that has received a lot attention is normalizing flows, which model distributions as pushforwards of a standard Gaussian through an \emph{invertible} neural network $G$. Thus, the likelihood has an explicit form via the change of variables formula using the Jacobian of $G$. 

Training normalizing flows is challenging due to a couple of main issues. Empirically, these models seem to require a much larger size than other generative models (e.g. GANs) and most notably, a much larger depth. This makes training challenging due to vanishing/exploding gradients. 
A very related problem is  \emph{conditioning}, more precisely the smallest singular value of the forward map $G$. It's intuitively clear that natural images will have a low-dimensional structure, thus a close-to-singular $G$ might be needed. On the other hand, the change-of-variables formula involves the determinant of the Jacobian of $G^{-1}$, which grows larger the more singular $G$ is.  

While recently, the universal approximation power of various types of invertible architectures has been studied \citep{dupont2019augmented,huang2020augmented} if the input is padded with a sufficiently large number of all-0 coordinates, precise quantification of the cost of invertibility in terms of the depth required and the conditioning of the model has not been fleshed out. 

In this paper, we study both mathematically and empirically representational aspects of depth and conditioning in normalizing flows and answer several fundamental questions. 

%The reasons for this, at least intuitively, are partially due to the weaker modeling power of the invertible transformations a flow model applies, and partially due to the fact that flow models use likelihood training, which amounts to fitting the input data in KL divergence; GANs on the other hand capture weaker metrics due to the limited power of the discriminators. 

%This tradeoff, though prevalent, has not been quantitatively formalized, much less mathematically fleshed out. In this paper, we focus on the representational aspect and formally tackle several fundamental questions about the representational power difference between common architectures for flow models and GANs. 
\section{Overview of Results} 

%We will formally present the results we will prove. First, we focus on results pertaining to depth.  

\subsection{Results about General Architectures} 

The most basic question about normalizing flows we can ask is how restrictive the assumption on invertibility of a model is---in particular how much the depth must increase to compensate for it. More precisely, we ask:   

{\bf Question 1:} is there a distribution over $\mathbb{R}^d$ which can be written as the pushforward of a Gaussian through a small, shallow generator, which cannot be written as the pushforward of a Gaussian through a small, shallow \emph{invertible} neural network? %(that is, a network in which each layer is a full rank $d \times d$ matrix, and the non-linearities used are invertible)?

Given that there is great latitude in terms of the choice of layer architecture, while keeping the network invertible, the most general way to pose this question is to require each layer to be a function of $p$ parameters -- i.e.    
$f = f_1 \circ f_2 \circ \cdots \circ f_{\ell}$
where $\circ$ denotes function composition and each $f_i : \mathbb{R}^d \to \mathbb{R}^d$ is an invertible function specified by a vector $\theta_i \in \mathbb{R}^p$ of parameters. 

This framing is extremely general: for instance it includes \emph{layerwise invertible feedforward networks} %of depth $\ell$
%with $p$ parameters per layer, i.e.  
in which $f_i(x) = \sigma^{\otimes d}(A_i x + b_i)$, $\sigma$ is invertible, $A_i \in \mathbb{R}^{d \times d}$ is invertible, $\theta_i = (A_i,b_i)$ and $p = d(d + 1)$.
It also includes popular architectures based on \emph{affine coupling blocks} (e.g. \cite{dinh2014nice, dinh2016density, kingma2018glow}) where each $f_i$ has the form  $f_i(x_{S_i}, x_{[d] \setminus S_i}) = (x_{S_i}, x_{[d] \setminus S_i} \odot g_i(x_{S_i}) + h_i(x_{S_i}))$
%\label{eq:affineblock} \end{equation}
%\end{definition}
for some $S \subset [d]$ which we revisit in more detail in the following subsection.  

% For example, for layerwise invertible GANs we would consider 

We answer this question in the negative: namely, we show that there is a distribution over $\mathbb{R}^d$ which can be expressed as the pushforward of a network with depth $O(1)$ and size $O(k)$ that cannot be (even very approximately) expressed as the pushforward of a Gaussian through a Lipschitz invertible network of depth smaller than $k/p$. 



%First we precisely define the class of networks we consider. Our lower bound is general and will apply to both the standard invertible GAN architecture as well as normalizing flow architectures like RealNVP; we state a general formulation of the result which encapsulates all of these and explain how to specialize it after the Theorem statement.


%single layer neural network of the form $f_i(x) = \sigma^{\otimes d}(A_i x + b_i)$, $\sigma$ is invertible, and $A_i$ is invertible. 

Towards formally stating the result, let $\theta = (\theta_1,\ldots,\theta_{\ell}) \in \Theta \subset \mathbb{R}^{d'}$  be the vector of all parameters (e.g. weights, biases) in the network, where $\theta_i \in \mathbb{R}^p$ are the parameters that correspond to layer $i$, and let $f_{\theta} : \mathbb{R}^d \to \mathbb{R}^d$ denote the resulting function. Define $R$ so that $\Theta$ is contained in the Euclidean ball of radius $R$. 

%Instead of assuming bounds on the size of individual parameters, we make the following more general assumption: let $\Theta \subset \mathbb{R}^{d'}$ be the set of parameters we consider,
%$f_{\theta} :\mathbb{R}^d \to \mathbb{R}^d$  parameterized by $\theta \in \mathbb{R}^{d'}$ 
We say the family $f_{\theta}$ is $L$-\emph{Lipschitz with respect to its parameters and inputs}, if 
$$\forall \theta, \theta ' \in \Theta: \E_{x \sim \mathcal N(0,I_{d \times d})} \|f_{\theta}(x) - f_{\theta'}(x)\|\leq L \|\theta - \theta'\| $$
and $\forall x,y \in \mathbb{R}^d, \|f_{\theta}(x) - f_{\theta}(y)\| \le L \|x - y\|$. \footnote{Note for architectures having trainable biases in the input layer, these two notions of Lipschitzness should be expected to behave similarly.}
%The second assumption is Lipschitzness in terms of the input, which behaves similarly to Lipschitzness in parameters for standard neural net architectures.
%Note this is somewhat different that the typical notion of Lipschitzness of the function itself in terms of its inputs.  
We will discuss the reasonable range for $L$ in terms of the weights after the Theorem statement.
%(Note that we can handle the case where $\sigma$ is $O(1)$-Lipschitz, by rescaling $\sigma$ and $A$ to reduce to the above case. Also, popular activations in practice like LeakyReLU and $\tanh$ are indeed Lipschitz.)
%Note that the composed function $f$ is then $L^{\ell}$ Lipschitz.
We show:
\begin{theorem} For every $d \in \mathbb{N}, \sigma > 0$ and $k = \exp(o(d)), L = \exp(o(d)), R = \exp(o(d))$, there exists a neural network $g: \mathbb{R}^d \to \mathbb{R}^d$ with $O(k)$ parameters and depth $O(1)$, s.t. for any family $\{f_{\theta}, \theta \in \Theta\}$ of layerwise invertible networks that are $L$-Lipschitz with respect to its parameters and inputs and $\Theta$ is contained in a ball of radius $R$, have $p$ parameters per layer and depth at most $k/p$ we have 
$$\forall \theta \in \Theta, W_1((f_{\theta})_{\# \mathcal{N}}, g_{\#\mathcal{N}}) \geq 10 \sigma^2 d$$
Furthermore, for all $\theta \in \Theta,$  
$ \mbox{KL}((f_{\theta})_{\# \mathcal{N}}, g_{\#\mathcal{N}}) \geq 1/10$ and  $\mbox{KL}(g_{\# \mathcal{N}}, (f_{\theta})_{\#\mathcal{N}}) \geq \frac{10 \sigma^2 d}{L^2} $. 

\label{l:sizedepth}
\end{theorem} 

\begin{comment}
\begin{theorem}
For every $d \in \mathbb{N}, \sigma > 0$ and $k = o(d^3)$, %$k = o(\exp(d))$,
there exists a neural network $g: \mathbb{R}^d \to \mathbb{R}^d$ with $O(k)$ parameters, s.t.  
for every layerwise invertible  $f: \mathbb{R}^d \to \mathbb{R}^d$ of depth $\ell$ at most $k/d^2$ we have 
$$W_1(f_{\# \mathcal{N}}, g_{\#\mathcal{N}}) \geq 10 \sigma^2 d$$
Furthermore, we also have 
$$ \mbox{KL}(f_{\# \mathcal{N}}, g_{\#\mathcal{N}}) \geq 1/10,  \hspace{0.5cm} \mbox{KL}(g_{\# \mathcal{N}}, f_{\#\mathcal{N}}) \geq \frac{10 \sigma^2 d}{L^2} $$ 
\end{theorem}
\end{comment}
\begin{comment}
For notational convenince, we'll say that a family of functions $f_{\theta} :\mathbb{R}^d \to \mathbb{R}^d$  parameterized by $\theta \in \mathbb{R}^{d'}$ is $L$-\emph{Lipschitz with respect to its parameters}, if 
$$\forall \theta, \theta ' \in \mathbb{R}^{d'}, \forall x \in \mathbb{R}^d: \|f_{\theta}(x) - f_{\theta'}(x)\|\leq L \|\theta - \theta'\|  $$ 


Then, we show: 

\begin{theorem} For every $d \in \mathbb{N}, \sigma > 0$ and $k = o(\exp(d)), L = o(\exp(d))$, there exists a neural network $g: \mathbb{R}^d \to \mathbb{R}^d$ with $O(k)$ parameters, s.t.  
for every layerwise invertible  $f: \mathbb{R}^d \to \mathbb{R}^d$ of depth at most $k/d^2$ (as defined in Question 1 above), which is an $L$-Lipschitz function with respect to its parameters, we have 
$$W_1(f_{\# \mathcal{N}}, g_{\#\mathcal{N}}) \geq 10 \sigma^2 d$$
Furthermore, we also have 
$$ \mbox{KL}(f_{\# \mathcal{N}}, g_{\#\mathcal{N}}) \geq 1/10,  \hspace{0.5cm} \mbox{KL}(g_{\# \mathcal{N}}, f_{\#\mathcal{N}}) \geq \frac{10 \sigma^2 d}{L^2} $$ 
\label{l:sizedepth}
\end{theorem} 
\end{comment}
We make several comments. First, note that while the number of parameters in both networks is comparable (i.e. it's $\Theta(k)$), the invertible network is deeper, which usually is accompanied with algorithmic difficulties for training, due to vanishing and exploding gradients. For layerwise invertible generators, if we assume that the nonlinearity $\sigma$ is $1$-Lipschitz and each matrix in the network has operator norm at most $M$, then a depth $\ell$ network will have $L = O(M^{\ell})$\footnote{Note, our theorem applies to exponentially large Lipschitz constants.} and $p = \Theta(d^2)$. For an affine coupling network with $g,h$ parameterized by $H$-layer networks with $p/2$ parameters each, $1$-Lipschitz activations and weights bounded by $M$ as above, we would similarly have $L = O(M^{\ell H})$.

We furthermore make several remarks on the ``hard'' distribution $g$ we construct, as well as the meaning of the parameter $\sigma$ and how to interpret the various lower bounds in the different metrics. The distribution $g$ for a given $\sigma$ will in fact be close to a mixture of $k$ Gaussians, each with mean on the sphere of radius $10 \sigma^2 d$ and covariance matrix $\sigma^2 I_d$. Thus -- this distribution has most of it's mass in a sphere of radius $O(\sigma^2 d)$---thus this is close to a trivial approximation for $g$. 

The KL divergence bounds are derived by so-called transport inequalities between KL and Wasserstein for subgaussian distributions \citep{bobkov1999exponential}. The discrepancy between the two KL divergences comes from the fact that the functions $g, f_{\theta}$ may have different Lipschitz constants, hence the tails of $g_{\# \mathcal{N}}$ and $f_{\# \mathcal{N}}$ behave differently. In fact, if the function $f_{\theta}$ had the same Lipschitz constant as $g$, both KL lower bounds would be on the order of a constant. 


\subsection{Results About Affine Coupling Architectures} Next, we prove several results for a particularly common normalizing flow architectures: those based on affine coupling layers \citep{dinh2014nice, dinh2016density, kingma2018glow}. The appeal of these architecture comes from training efficiency. Although layerwise invertible neural networks (i.e. networks for which each layer consists of an invertible matrix and invertible pointwise nonlinearity) seem like a natural choice, in practice this is computationally prohibitive. 

Concretely, if a random variable $z$ has a probability density function $\phi(z)$ and distribution $p$ is the pushforward of the $z$ through an invertible function $f$, the density of $p$ at a point $x$ is $\displaystyle p(x) = \phi(f^{-1}(x)) |\mbox{det}(J_f(f^{-1}(x)))|^{-1}$, where $J_f$ denotes the Jacobian of the function $f$. Hence, maximizing the likelihood of the observable data requires an efficient way of evaluating the determinant of the Jacobian of $f$. For a structurally unrestricted network, the determinant of the Jacobian for such networks will be a $\Theta(d^3)$ operation, which is prohibitively expensive. 

Consequently, it's typical for the transformations in a flow network to be constrained in a manner that allows for efficient computation of the Jacobian determinant. The most common building block is an \emph{affine coupling} block, originally proposed by \cite{dinh2014nice, dinh2016density}. A coupling block partitions the coordinates $[d]$ into two parts: $S$ and $[d] \setminus S$, for a subset $S$ with $|S|$ containing around half the coordinates of $d$. The transformation then has the form: 
\begin{definition} An \emph{affine coupling block} is a map $f: \mathbb{R}^d \to \mathbb{R}^d$, s.t.   
$f(x_S, x_{[d] \setminus S}) = (x_S, x_{[d] \setminus S} \odot g(x_S) + h(x_S))$ \label{eq:affineblock} %\end{equation}
\end{definition}
Of course, the modeling power will be severely constrained if the coordinates in $S$ never change: so typically, flow models either change the set $S$ in a fixed or learned way (e.g. alternating between different partitions of the channel in \cite{dinh2016density} or applying a learned permutation in \cite{kingma2018glow}). Of course, a permutation is a discrete object, so difficult to learn in a differentiable manner -- so  \cite{kingma2018glow} simply learns an invertible linear function (i.e. a 1x1 convolution) as a differentiation-friendly relaxation thereof.  

\subsubsection{The effect of choice of partition on depth} 

The first question about affine couplings we ask is how much of a saving in terms of the depth of the network can one hope to gain from using learned partitions (ala GLOW) as compared to a fixed partition. More precisely: 

{\bf Question 2:} Can models like Glow \citep{kingma2018glow} be simulated by a sequence of affine blocks with a fixed partition without increasing the depth by much? 

We answer this question in the affirmative at least for equally sized partitions (which is what is typically used in practice). We show the following surprising fact: consider an arbitrary partition $(S, [2d] \setminus S)$ of $[2d]$, such that $S$ satisfies $|S| = d$, for $d \in \mathbb{N}$. Then for any invertible matrix $T \in \mathbb{R}^{2d \times 2d}$, the linear map $T: \mathbb{R}^{2d} \to \mathbb{R}^{2d}$ can be exactly represented by a composition of $O(1)$ affine coupling layers that are \emph{linear}, namely have the form $L_i(x_S, x_{[2d]\setminus S}) = (x_S, B_i x_{[2d] \setminus S} + A_i x_S)$ or $L_i(x_S, x_{[2d]\setminus S}) = (C_i x_{S} + D_i x_{[2d] \setminus S}, x_{[2d] \setminus S})$
for matrices $A_i, B_i, C_i, D_i\in \mathbb{R}^{d\times d}$, s.t. each $B_i, C_i$ is diagonal. For convenience of notation, without loss of generality let $S = [d]$. Then, each of the layers $L_i$ is a matrix of the form $\begin{bmatrix}I & 0\\ A_i & B_i\end{bmatrix}$ or $\begin{bmatrix} C_i & D_i\\ 0 & I\end{bmatrix}$, where the rows and columns are partitioned into blocks of size $d$. 

With this notation in place, we show the following theorem: 
%In order to do that, we'll consider couplings of linear functions of the form
%with $B_i, C_i$ diagonal. The main theorem is as follows:
\begin{theorem}
\label{thm:linear_simulation_main}
For all $d\in\mathbb{N}$, there exists a $K \leq 47$ such that for any invertible $T \in \R^{2d \times 2d}$ with $\mbox{det}(T)>0$, there exist matrices $A_{i}, D_{i}\in \R^{d\times d}$ and diagonal matrices $B_{i}, C_{i}\in \R_{\ge 0}^{d\times d}$ for all $i \in [k]$ such that
\[T = \prod_{i=1}^{K}\begin{bmatrix}I & 0\\ A_i & B_i\end{bmatrix} \begin{bmatrix}C_i & D_i\\ 0 & I\end{bmatrix} \]
\end{theorem}
%\Anote{statement needs updating}\Vnote{updated the statement and commentary above, check}

In particular, since permutation matrices are invertible, this means that any applications of permutations to achieve a different partition of the inputs (e.g. like in Glow \citep{kingma2018glow}) can in principle be represented as a composition of not-too-many affine coupling layers, indicating that the flexibility in the choice of partition is not the representational bottleneck.

It's a reasonable to ask how optimal the $K = 47$ bound is -- we supplement our upper bound with a lower bound, namely that $K \ge 5$. This is surprising, as naive parameter counting would suggest $K = 4$ might work. Namely, we show: 

\begin{theorem}
\label{thm:linear_lower_main}
For all $d\in\mathbb{N}$ and $K \le 4$, there exists an invertible $T \in \R^{2d \times 2d}$ with $\mbox{det}(T)>0$, s.t. for all $A_{i}, D_{i}\in \R^{d\times d}$ and for all diagonal matrices $B_{i}, C_{i}\in \R_{\ge 0}^{d\times d}, i \in [k]$ it holds that
\[T \neq \prod_{i=1}^{K}\begin{bmatrix}I & 0\\ A_i & B_i\end{bmatrix} \begin{bmatrix}C_i & D_i\\ 0 & I\end{bmatrix} \]
\end{theorem}

Beyond the relevance of this result in the context of how important the choice of partitions is, it also shows a lower bound on the depth for an equal number of \emph{nonlinear} affine coupling layers (even with quite complex functions $s$ and $t$ in each layer) -- since a nonlinear network can always be linearized about a (smooth) point to give a linear network with the same number of layers.
In other words, studying linear affine coupling networks lets us prove a \emph{depth lower bound}/\emph{depth separation} for nonlinear networks for free.


%Furthermore, any affine coupling network built out of piecewise smooth functions can be linearized around a smooth point, so a lower bound for the ability of linear networks to represent a linear function also implies the corresponding lower bound on the depth for an equal number of nonlinear affine coupling layers (even with quite complex functions $s$ and $t$ in each layer). In other words, studying linear affine coupling networks lets us prove a \emph{depth lower bound}/\emph{depth separation} for nonlinear networks for free.



Finally, in Section \ref{l:explin}, we include an empirical investigation of our theoretical results on synthetic data, by fitting random linear functions of varying dimensionality with linear affine networks of varying depths in order to see the required number of layers. The results there suggest that the constant in the upper bound is quite loose -- and the correct value for $K$ is likely closer to the lower bound -- at least for random matrices.

\subsubsection{Universal Approximation with Ill-Conditioned Affine Coupling Networks}  

Finally, we turn to universal approximation and the close ties to conditioning. Namely, a recent work (Theorem 1 of \citep{huang2020augmented}) showed that deep affine coupling networks are universal approximators if we allow the training data to be padded with sufficiently many zeros. While zero padding is convenient for their analysis (in fact, similar proofs have appeared for other invertible architectures like Augmented Neural ODEs \citep{zhang2020approximation}), in practice models trained on zero-padded data often perform poorly (see Appendix~\ref{a:experiments}). 

In fact, we show that neither padding nor depth is necessary representationally: shallow models without zero padding are already universal approximators in Wasserstein. 
\begin{theorem}[Universal approximation without padding]\label{thm:universal-no-padding}
Suppose that $P$ is the standard Gaussian measure in $\mathbb{R}^n$ with $n$ even and $Q$ is a distribution on $\mathbb{R}^n$ with bounded support and  absolutely continuous with respect to the Lebesgue measure. Then for any $\epsilon > 0$, there exists a depth-3 affine coupling network $g$, with maps $s,t$ represented by feedforward ReLU networks such that $W_2(g_{\#} P, Q ) \le \epsilon$.
\end{theorem}

A shared caveat of the universality construction in Theorem~\ref{thm:universal-no-padding} with the construction in \cite{huang2020augmented} is that the resulting network is poorly conditioned. In the case of the construction in \cite{huang2020augmented}, this is obvious because they  pad the $d$-dimensional training data with $d$ additional zeros, and a network that takes as input a Gaussian distribution in $\mathbb{R}^{2d}$ (i.e. has full support) and outputs data on $d$-dimensional manifold (the space of zero padded data) must have a singular Jacobian almost everywhere.\footnote{Alternatively, we could feed a degenerate Gaussian supported on a $d$-dimensional subspace into the network as input, but there is no way to train such a model using maximum-likelihood training, since the prior is degenerate.} In the case of Theorem~\ref{thm:universal-no-padding}, the condition number of the network blows up at least as quickly as $1/\epsilon$ as we take the approximation error $\epsilon \to 0$, so this network is also ill-conditioned if we are aiming for a very accurate approximation. Based on Theorem~\ref{thm:linear_lower_main}, we can show that condition number blowup of either the Jacobian or the Hessian is necessary for such a shallow model to be universal, even when approximating well-conditioned linear maps (see Remark~\ref{rmk:linear-vs-universal}). %(Section~\ref{a:experiments}).
%\Anote{Fred: I'm not quite sure I get the last sentence, can you expand?}

%\Anote{More writing about experiments needed here}\Vnote{decided that I would talk about what we did for the tanh thing and for the PLN thing right after the theory stuff for each. feel free to reorganize}
%be written as the pushforward of a Gaussian through a small GAN that cannot be approximated by a very powerful architecture---either when the depth is allowed to be very large, or when the non-linearities are allowed to be very rich? 



%Next, we consider architectures based on affine couplings. On the side of limitations, we first show that regardless of the choice of how the partitions $S$ are chosen, an iterated sequence of affine coupling blocks with $\tanh$ nonlinearities cannot exactly represent even an entrywise application of $\tanh$. Namely, we show:    



%\begin{theorem}[Large Depth doesn't Help] 
%Consider the function $g: \mathbb{R}^d \to \mathbb{R}^d, g(z) = (\tanh{z_1}, \dots,  \tanh{z_d})$. The function $g$ cannot be exactly represented as an iterated sequence of affine coupling blocks of the form 
%$$(z_S, z_{\bar{S}}) \to (z_S, z_{\bar{S}} \odot %f(z_S) + g(z_S))$$ 
%where $f$ and $g$ are arbitrarily (full-connected) $\tanh$ neural networks,
%regardless of the number of layers or the choice of subsets $S \subseteq [d]$ for the layers.  
%\end{theorem} 


\begin{comment}
Turning to the aspect of the power of the nonlinearities -- we show that the structural assumption of the affine block itself provides a non-trivial representational restriction: even if the power of the non-linear transformations in an affine coupling block is essentially unbounded (i.e. they can be arbitrary smooth funcions), a small number of such blocks cannot represent pushforwards of moderately sized generative networks. Precisely, we show: 

\begin{theorem}[Large Width Doesn't Help] 
 There exists a neural network $g: \mathbb{R}^d \to \mathbb{R}^d$ with $2^{d/2}$ \Anote{slightly more} parameters \Anote{Lipschitz, nonlinearity?}, s.t. for every neural network $f$, s.t. each layer of $f$ has the form 
$$(z_S, z_{\bar{S}}) \to (z_S, z_{\bar{S}} \odot f(z_S) + g(z_S))$$
for a subset $S$, s.t. $|S| = d/2$ and is $L$-lipschitz, we have 
 $$W_1(f_{\# \mathcal{N}}, g_{\#\mathcal{N}}) \geq ??$$ 
\end{theorem}
\end{comment}




==> old_related_work.tex <==
\vspace{-0.2cm}
\section{Related Work}
\vspace{-0.2cm}
On the empirical side, flow models were first popularized by \cite{dinh2014nice}, who introduce the NICE model and the idea of parametrizing a distribution as a sequence of transformations with triangular Jacobians, so that maximum likelihood training is tractable. Quickly thereafter,  \cite{dinh2016density} improved the affine coupling block architecture they introduced to allow non-volume-preserving (NVP) transformations, and finally \cite{kingma2018glow} introduced 1x1 convolutions in the architecture, which they view as relaxations of permutation matrices---intuitively, allowing learned partitions for the affine blocks.  Subsequently, there have been variants on these ideas: \citep{grathwohl2018ffjord, dupont2019augmented, behrmann2018invertible} viewed these models as discretizations of ODEs and introduced ways to approximate determinants of non-triangular Jacobians, though these models still don't scale beyond datasets the size of CIFAR10. The conditioning/invertibility of trained models was experimentally studied in \citep{behrmann2019invertibility}, along with some ``adversarial vulnerabilities'' of the conditioning.
Mathematically understanding the relative representational power and statistical/algorithmic implications thereof for different types of generative models is still however a very poorly understood and nascent area of study. 

Most closely related to our results are the recent works of \cite{huang2020augmented} and \cite{zhang2020approximation}. Both prove universal approximation results for invertible architectures (the former affine couplings, the latter neural ODEs) if the input is allowed to be padded with zeroes. As already expounded upon in the previous sections -- our results prove universal approximation even without padding, but we focus on more fine-grained implications to depth and conditioning of the learned model. % ADDED 10/13 TO ARXIV RELATED_WORK
Another work \citep{kong2020expressive} studies the representational power of Sylvester and Householder flows, normalizing flow architectures which are quite different from affine coupling networks. In particular, they prove a depth lower bound for local planar flows with bounded weights; for planar flows, our general Theorem~\ref{l:sizedepth} can also be applied, but the resulting lower bound instances are very different (ours targets multimodality, theirs targets tail behavior).

More generally, there are various classical results that show a particular family of generative models can closely approximate most sufficiently regular distributions over some domain. Some examples are standard results for mixture models with very mild conditions on the component distribution (e.g. Gaussians, see \citep{everitt2014finite}); Restricted Boltzmann Machines and Deep Belief Networks  \citep{montufar2011expressive, montufar2011refinements}; GANs  \citep{bailey2018size}. 

%Separation results between different families/architectures of distributions are much harder, and results here are few and far between. \cite{lee2017ability} showed certain separations in the setting of GANs: namely, that there deep generators where each layer satisfies certain Fourier properties that cannot be approximately expressed as shallower generators in the Wasserstein sense.  


%In the simpler function approximation setting, where we merely care about approximating functions, rather than distributions, a bit more has been done in recent years. For instance, in the setting of neural networks, a question of particular interest is the benefit conferred by depth. A seminal result by \cite{telgarsky2016benefits} showed that there are small, but deep neural networks that cannot be approximated by a small, shallow neural networks (a substantial number of papers of similar flavor followed \cite{eldan2016power, raghu2017expressive, chatziafratis2019depth}). 
%Somewhat related to our results are also results due to \cite{lu2017expressive, hanin2017approximating} which show that narrow (of width at most the dimension of the input) neural networks are not universal approximators, but slightly wider neural networks are.  
%\Anote{I feel like this may be a bit too lengthy -- we can probably cut the last 3 paragraphs or shorten a lot.}
%\Anote{To add: gaussanization flows, universal approximation of ODEs}


==> universality_apdx.tex <==
\section{Appendix for Section~\ref{sec:universality}}
%In recent work \cite{?}, it was shown using a sophisticated proof that affine coupling networks are universal approximators in Wasserstein distance if we allow the number of affine coupling layers used and the size of the $s$ and $t$ networks to go to infinity, and also allow the output of the network to be zero-padded. A practical concern with this result (besides the very large width and depth the proof requires) is that training with zero-padding empirically performs very badly, much worse than without padding (see experiments); intuitively this is because the Jacobian will need to explode if we try to approach the optimal transport map.

%Because of the practical concerns about degenerate Jacobians, we believe the other results in this paper are more relevant to the use of affine coupling networks in practice (and this is supported by the experiments). Nevertheless for completeness, we record a couple ways in which the previous theoretical result of \cite{?} can be improved. 

\paragraph{Simpler universality under zero-padding.} First (as a warmup), we give a much simpler proof than \cite{huang2020augmented} that affine coupling networks are universal approximators in Wasserstein under zero-padding, which moreover shows that only a small number of affine coupling layers are required. For $Q$ a probability measure over $\mathbb{R}^n$ satisfying weak regularity conditions (see Theorem~\ref{thm:brenier} below), by Brenier's Theorem \cite{villani2003topics} there a $W_2$ optimal transport map
\[ \varphi : \mathbb{R}^n \to \mathbb{R}^n \]
such that if $X \sim N(0,I_{n \times n})$, then the pushforward $\varphi_{\#}(X)$ is distributed according to $Q$, and a corresponding transport map in the opposite direction which we denote $\varphi^{-1}$. If we allow for arbitrary functions $t$ in the affine coupling network, then we can implement the zero-padded transport map $(X,0) \mapsto (\varphi(X),0)$ as follows:
\begin{equation}\label{eqn:zero-padding-map}
(X,0) \mapsto (X, \varphi(X)) \mapsto (\varphi(X),\varphi(X)) \mapsto (\varphi(X),0).
\end{equation}
Explicitly, in the first layer the translation map is $t_1(x) = \varphi(x)$, in the second layer the translation map is $t_2(x) = x - \varphi^{-1}(x)$, and in the third layer the translation map is $t_3(x) = -x$. Note that no scaling maps are required: with zero-padding the basic NICE architecture can be universal, unlike in the unpadded case where NICE can only hope to implement volume preserving maps. This is because every map from zero-padded data to zero-padded data is volume preserving. Finally, if we are required to implement the translation maps using neural networks, we can use standard approximation-theoretic results for neural networks, combined with standard results from optimal transport, to show universality of affine coupling networks in Wasserstein. First, we recall the formal statement of Brenier's Theorem:
\begin{theorem}[Brenier's Theorem, Theorem 2.12 of \cite{villani2003topics}]\label{thm:brenier}
Suppose that $P$ and $Q$ are probability measures on $\mathbb{R}^n$ with densities with respect to the Lebesgue measure. Then $Q = (\nabla \psi)_{\#} P$ for $\psi$ a convex function, and moreover $\nabla \psi$ is the unique $W_2$-optimal transport map from $P$ to $Q$.
\end{theorem}
\iffalse
\begin{theorem}[\cite{caffarelli1992regularity}]
Suppose that $P,Q$ are as in Theorem~\ref{thm:brenier}, and furthermore $P$ is supported on a bounded subset $\Omega_1 \subset \mathbb{R}^n$ with a density $f_1$ on this set bounded away from 0 and infinity, and $Q$ is supported on a bounded convex subset $\Omega_2 \subset \mathbb{R}^n$ with a density $f_2$ bounded away from 0 and infinity. If $f_1,f_2 \in C^{\overline{a}}$ then 
\end{theorem}
\fi
It turns out that the transportation map $\varphi := \nabla \psi$ is not always a continuous function, however there are simple sufficient conditions for the distribution $Q$ under which the map is continuous (see e.g. \cite{caffarelli1992regularity}). From these results (or by directly smoothing the transport map), we know any distribution with bounded support can be approached in Wasserstein distance by smooth pushforwards of Gaussians. So for simplicity, we state the following Theorem for distributions which are the pushforward of smooth maps.
\begin{theorem}[Universal approximation with zero-padding]\label{thm:universal-zero}
Suppose that $P$ is the standard Gaussian measure in $\mathbb{R}^n$ and $Q = \varphi_{\#} P$ is the pushforward of the Gaussian measure through $\varphi$ and $\varphi$ is a smooth map. Then for any $\epsilon > 0$ there exists a depth 3 affine coupling network $g$ with no scaling and feedforward ReLU net translation maps such that $W_2(g_{\#} (P \times \delta_{0^n}), Q \times \delta_{0^n}) \le \epsilon$.
\end{theorem}
\begin{proof}
For any $M > 0$, let $f_M(x) = \min(M, \max(-M, x))$ be the 1-dimensional truncation map to $[-M,M]$ and for a vector $x \in \mathbb{R}^n$ let $f_M(x) \in [-M,M]^n$ be the result of applying $f_M$ coordinate-wise. Note that $f_M$ can be implemented as a ReLU network with two hidden units per input dimension. Also, any continuous function on $[-M,M]^n$ can be approximated arbitrarily well in $L^{\infty}$ by a sufficiently large ReLU neural network with one hidden layer \cite{leshno1993multilayer}. Finally,  note that if $\|f - g\|_{L^{\infty}} \le \epsilon$ then for any distribution $P$ we have $W_2(f_{\#} P, g_{\#} P) \le \epsilon$ by considering the natural coupling that feeds the same input into $f$ and $g$.

Now we show how to approximate the construction of \eqref{eqn:zero-padding-map} using these tools. For any $\epsilon > 0$, if we choose $M$ sufficiently large and then take $\tilde{\varphi}$ and $\widetilde{\varphi^{-1}}$ to be sufficiently good approximations of $\varphi$ and $\varphi^{-1}$ on $[-M,M]^n$, we can construct an affine coupling network with ReLU feedforward network translation maps $\tilde{t}_1(x) = f_M(\tilde{\varphi}(f_M(x)))$, $\tilde{t}_2(x) = x - \widetilde{\varphi^{-1}}(x)$, and $\tilde{t}_3(x) = -x$, such that the output has $W_2$ distance at most $\epsilon$ from $Q$.
%\[ (X,0) \mapsto (X, t_M(\tilde\varphi(t_M(X)))) \mapsto (\]
\end{proof}

\paragraph{Universality without padding.} We now show that universality in Wasserstein can be proved even if we don't have zero-padding, using a lattice-based encoding and decoding scheme. Let $\epsilon > 0$ be a small constant, to be taking sufficiently small. Let $\epsilon' \in (0,\epsilon)$ be a further constant, taken sufficiently small with respect to $\epsilon$ and similar for $\epsilon''$ wrt $\epsilon'$. Suppose the input dimension is $2n$, and let $X = (X_1,X_2)$ with independent $X_1 \sim N(0,I_{n \times n})$ and $X_2 \sim N(0,I_{n \times n})$ be the input the the affine coupling network. Let $f(x)$ be the map which rounds $x \in \mathbb{R}^n$ to the closest grid point in $\epsilon \mathbb{Z}^n$ and define $g(x) = x - f(x)$. Note that for a point of the form $z = f(x) + \epsilon' y$ for $y$ which is not too large, we have that $f(z) = f(x)$ and $g(z) = y$. Let $\varphi_1,\varphi_2$ be the desired orientation-preserving maps (fixme: details). 
Now we consider the following sequence of maps:
\begin{align} 
(X_1,X_2) &\mapsto (X_1, \epsilon' X_2 + f(X_1)) \label{eqn:f1}
\\
&\mapsto (f(\varphi_1(f(X_1),X_2)) + \epsilon' \varphi_2(f(X_1),X_2) + O(\epsilon''), \epsilon' X_2 + f(X_1)) \label{eqn:f2}\\
&\mapsto (f(\varphi_1(f(X_1),X_2)) + \epsilon' \varphi_2(f(X_1),X_2) + O(\epsilon''), \varphi_2(f(X_1),X_2) + O(\epsilon''/\epsilon')). \label{eqn:f3}
\end{align}
More explicitly, in the first step we take $s_1(x) = \log(\epsilon') \vec{1}$ and $t_1(x) = f(x)$. In the second step, we take $s_2(x) = \log(\epsilon'') \vec{1}$ and $t_2$ is defined by $t_2(x) = f(\varphi_1(f(x),g(x))) + \epsilon' \varphi_2(f(x),g(x))$. In the third step, we take $s_3(x) = \log(\epsilon'') \vec{1}$ and define $t_3(x) = \frac{g(x)}{\epsilon'}$.

Again, taking sufficiently good approximations to all of the maps allows to approximate this map with neural networks, which we formalize below. %(Note that while $f$ is not continuous, it is continuous almost everywhere and it can be modified to be continuous by convolution with an appropriate bump function.)

%\begin{theorem}[Universal approximation without padding]
%Suppose that $P$ is the standard Gaussian measure in $\mathbb{R}^n$ and $Q = \varphi_{\#} P$ is the pushforward of the Gaussian measure through $\varphi$ and $\varphi$ is a smooth map. Then for any $\epsilon > 0$ there exists a depth 3 affine coupling network $g$ with feedforward ReLU net scaling and translation maps such that $W_2(g_{\#} P, Q ) \le \epsilon$.
%\end{theorem}
\begin{proof}[Proof of Theorem~\ref{thm:universal-no-padding}
Turning \eqref{eqn:f1},\eqref{eqn:f2}, and \eqref{eqn:f3} into a universal approximation theorem for ReLU-net based feedforward networks just requires to modify the proof of Theorem~\ref{thm:universal-zero} for this scenario.

Fix $\delta > 0$, the above argument shows we can choose $\epsilon,\epsilon',\epsilon'' > 0$ sufficiently small so that if $h$ is map defined by composing \eqref{eqn:f1},\eqref{eqn:f2}, and \eqref{eqn:f3}, then  $W_2(h_{\#} P, Q) \le \epsilon/4$. The layers defining $h$ may not be continuous, since $f$ is only continuous almost everywhere. Using that continuous functions are dense in $L^2$, we can find a function $f_{\epsilon}$ which is continuous and such that if we define $h_{\epsilon}$ by replacing each application of $f$ by $f_{\epsilon}$, then $W_2(h_{\epsilon}\# P, Q) \le \epsilon/2$. 

Finally, since $f_{\epsilon}$ is an affine coupling network with continuous $s$ and $t$ functions, we can use the same truncation-and-approximation argument from Theorem~\ref{thm:universal-zero} to approximate it by an affine coupling network $g$ with ReLU feedforward $s$ and $t$ functions such that $W_2(g\# P, Q) \le \epsilon$, which proves the result.
\end{proof}
